Video Generation Meets Agent Harness: Agentic Video Generation, Agentic World Modeling and Recursive Self-Improvement

Video generation is shifting from end-to-end synthesis toward agentic generation, where planning, tool use, and feedback enable coherent, controllable multi-shot videos. In parallel, video world models provide action-conditioned observations and predicted futures, serving as interactive environments for agents. We study their intersection through the agent harness: an executable runtime that constructs context, exposes tools, maintains state, routes feedback, and manages budgets around video models. This report examines three directions. First, agentic video generation, where harnesses coordinate scripting, shot planning, asset management, production, and editing, alongside the evaluation challenges of these systems. Second, agentic world modeling, where harnesses mediate observation, control, execution, and state. We discuss hybrid designs in which game engines or agent-written programs maintain world state while video models render observations, and how agents and world models can mutually evaluate and improve one another. Third, recursive self-improvement (RSI) in video model development, distinguishing output revisions, updates to harness state, generator parameters, and evaluators, and changes to the improvement procedure itself. We identify how these improvements feed back into subsequent development. Across these directions, we analyze essential agent capabilities, including audiovisual perception, long-horizon planning, memory, code-based interaction, feedback-guided control, skill reuse, and multi-agent coordination. We conclude with challenges in autonomous video production, lifelong memory, programmable hybrid control, autonomous model development, provenance, cost accounting, and evaluation linking video quality and task performance to sustained improvements in models and harnesses.

==> figures/taxonomy-fonts.tex <==
% Local font helpers: Arial figures and Times New Roman tables.
% XeLaTeX/LuaLaTeX can resolve this font by name locally and on Overleaf.
% Keep the manuscript's existing text, sans-serif, monospace and math fonts.
\RequirePackage{iftex}
\ifPDFTeX
  \newcommand{\SurveyTableFont}{\fontfamily{ptm}\selectfont}
  \newcommand{\TaxonomyArial}{\fontfamily{phv}\selectfont}
  \newcommand{\TaxonomySans}{\fontfamily{phv}\selectfont}
  \PackageWarningNoLine{taxonomy-fonts}{Times/Helvetica-compatible fallbacks active.
    Use XeLaTeX for exact Times New Roman and Arial}
\else
  \let\taxSavedEncodingDefault\encodingdefault
  \let\taxSavedRomanDefault\rmdefault
  \let\taxSavedSansDefault\sfdefault
  \let\taxSavedMonoDefault\ttdefault
  \let\taxSavedFamilyDefault\familydefault
  \RequirePackage[no-math]{fontspec}
  \newfontfamily\SurveyTableFont{Times New Roman}[Ligatures=TeX]
  \newfontfamily\TaxonomyArial{Arial}[Ligatures=TeX]
  % Match the existing class's 0.90-scaled Helvetica size: the root's nominal
  % 10 pt setting remains visually 9 pt when switching the face to Arial.
  \newfontfamily\TaxonomySans{Arial}[Ligatures=TeX,Scale=0.90]
  \let\encodingdefault\taxSavedEncodingDefault
  \let\rmdefault\taxSavedRomanDefault
  \let\sfdefault\taxSavedSansDefault
  \let\ttdefault\taxSavedMonoDefault
  \let\familydefault\taxSavedFamilyDefault
  \normalfont
\fi
% Scope this command to a table environment/group. The class resets font
% families in captions and bold text, so keep those local resets in TNR too.
\makeatletter
\newcommand{\SurveyTableSetup}{%
  % A longtable can ship the preceding page while this group is active.
  % Keep the class's footer size/style, but restore its original font family.
  \edef\SurveyTablePageFont{%
    \noexpand\fontencoding{\encodingdefault}%
    \noexpand\fontfamily{\familydefault}\noexpand\selectfont}%
  \let\SurveyTableSavedFooterFont\footerfont
  \def\footerfont{\SurveyTableSavedFooterFont\SurveyTablePageFont}%
  \SurveyTableFont
  \edef\encodingdefault{\f@encoding}%
  \edef\rmdefault{\f@family}%
  \edef\sfdefault{\f@family}%
  \edef\ttdefault{\f@family}%
  \edef\familydefault{\f@family}%
  \normalfont
}
\makeatother

